Unbiased Scene Graph Generation from Biased Training

Today's scene graph generation (SGG) task is still far from practical, mainly due to the severe training bias, e.g., collapsing diverse "human walk on / sit on / lay on beach" into "human on beach". Given such SGG, the down-stream tasks such as VQA can hardly infer better scene structures than merely a bag of objects. However, debiasing in SGG is not trivial because traditional debiasing methods cannot distinguish between the good and bad bias, e.g., good context prior (e.g., "person read book" rather than "eat") and bad long-tailed bias (e.g., "near" dominating "behind / in front of"). In this paper, we present a novel SGG framework based on causal inference but not the conventional likelihood. We first build a causal graph for SGG, and perform traditional biased training with the graph. Then, we propose to draw the counterfactual causality from the trained graph to infer the effect from the bad bias, which should be removed. In particular, we use Total Direct Effect (TDE) as the proposed final predicate score for unbiased SGG. Note that our framework is agnostic to any SGG model and thus can be widely applied in the community who seeks unbiased predictions. By using the proposed Scene Graph Diagnosis toolkit on the SGG benchmark Visual Genome and several prevailing models, we observed significant improvements over the previous state-of-the-art methods.

==> sections/6_abandoned.tex <==
\section{Model Zoo}
\label{sec:models}
For most of SGG methods~\cite{zellers2018neural, tang2019learning, yang2018graph, xu2017scene}, they mainly focus on how to extract or utilize object features while the proposed TDE analysis is a high-level inference strategy that is agnostic to how the models are implemented. Three models~\cite{zhang2017visual, zellers2018neural, tang2019learning} and two fusion functions that used in our experiments are all observed significant improvements after we apply TDE.

\noindent\textbf{VTransE}~\cite{zhang2017visual} assumes subjects, objects and predicates are all in the same latent space, using the translation vectors from subjects to objects as the embedded features of predicates. In other word, the relationship is considered as a feature translation, $subject + predicate \approx object$, rather than a triplet combination, $(subject, predicate, object)$. To be specific, the joint object feature $x'_{\varepsilon}$ in Module~\ref{module:3} is implemented as $x'_{\varepsilon}=FC_o(x_i) - FC_s(x_j)$. 

\noindent\textbf{MOTIFS}~\cite{zellers2018neural} encodes global structural patterns as additional information for local predictions. It uses bidirectional LSTMs in Module~\ref{module:1}~\ref{module:3}. Note that the object labels are also decoded by a LSTM layer in Module~\ref{module:2}, which takes both object feature and the previous softmax probability as input: $\hat{z}_i=Softmax(FC_z(LSTM([x_i;\hat{z}_{i-1}])))$, where the final label $z_i$ is the onehot version of $\hat{z}_i$.

\noindent\textbf{VCTree}~\cite{tang2019learning} is very similar to MOTIFS. The main difference is that Tree-LSTMs~\cite{tai2015improved} are used to better modeling the hierarchical nature of images. To generate tree structures, VCTree calculates a score matrix for each pair of objects measuring their probability to have a relationship. The binary version of maximum spanning tree is then constructed to guide the message passing of Tree-LSTMs.

\noindent\textbf{Fusion Functions} decide how different branches interact together to make a prediction of $Y$. We tested two simple functions, 1) weighted sum, and 2) gated multiplication, for all three models to justify the generalization ability of TDE. The details will be discussed in Section~\ref{sec:exp}.


% Despite recent progresses~\cite{xu2017scene, zellers2018neural, tang2019learning, chen2019scene, chen2019counterfactual, zhang2019graphical} that have been made in scene graph generation (SGG), existing SGG methods~\cite{zellers2018neural, chen2019counterfactual, zhang2019graphical} are usually biased towards ambiguous trivial relationships such as ``on'', ``near''. As shown in Figure~\ref{fig:1}, the biased scene graph (SG) neglects the more fine-grained relationships, ``parked on'', ``behind'' or ``in front of'', simply because their lower sampling fractions in the training set. Since the degraded predicates like ``on'' are not able to distinguish the specific visual relationships like ``man laying on bed'' and ``man sitting on bed'', it will lead to a serious consequence that such a biased SG only provides a sparse object structure rather than meaningful relationships to downstream tasks~\cite{johnson2018image, yang2019auto, teney2017graph}, which is against the original intention of SGG.

% To better understand the cause of biased SGG, we visualize the distribution of sampling fraction for the most frequent 20 predicates in VG dataset~\cite{krishna2017visual}. As we can see from Figure~\ref{fig:1}.b, top-10 predicates cover about 90\% samples in the dataset and most of them are trivial, or in other word, generalized predicates. We believe that it's partially caused by the bounded rationality~\cite{simon1990bounded} and reporting bias~\cite{misra2016seeing} of annotators. Bounded rationality and reporting bias indicate that when people make complicated decisions, they tend to give subjectively satisfactory solutions rather than optimal ones due to the attention span, limited time and other cognitive limitations. As a result, when making annotations from multiple candidate predicates, more generalized answers are easier to be selected. But more importantly, the long tail distribution of predicates is the nature of real world. For example, there are more spatial relationships like ``on'', ``under'', ``behind'' than semantic relationships like ``eating'', ``riding''.

% Bias problems have long been investigated in machine learning~\cite{torralba2011unbiased}. Existing debiasing methods can be roughly categorized into three types: 1) data augmentation or re-sampling~\cite{geirhos2018imagenettrained, li2018resound, li2019repair}, 2) unbiased learning through elaborately designed training curriculums or learning losses~\cite{zemel2013learning}, 3) disentangling biased representations from the unbiased~\cite{wang2018learning, Quadrianto_2019_CVPR}. However, even if we can identify where and what bias exists in SGG, it doesn't mean that we can perfectly eliminate them. For SGG, collecting unusual relationships is too expensive while other debiasing methods are easy to hurt the useful prior~\cite{lu2016visual, zellers2018neural}, which helps model filter most of the impossible relationships, \eg, ``apple parked on table'' or ``apple standing on table''.

% Note that the long tail problem naturally exists in real world, but how can our human intelligence learn from biased environment while conduct unbiased inferences? This is because memorizing and utilizing are essentially different in human learning process~\cite{biggs2014evaluating}. The case by case inference will help human beings identify and be free from the memorized population bias. Yet, conventional machine learning prediction doesn't explicitly distinguish the testing (utilizing) stage from training (memorizing) stage.  

% \textbf{Biased Prediction}: Take a biased SGG~\cite{zellers2018neural} in Figure~\ref{fig:1}.e as example, The Recall@k of each predicate is almost in direct proportion to their sampling fractions, which implies that the likelihood used during testing only reflects statistical prior of certain patterns in population rather than individually seeks optimal matching results, because most of the worse predicate performances are even not caused by hard categories.

% %Since patterns are still need to learn from population
% \textbf{Unbiased Prediction}: We respect the conventional likelihood based training as the memorizing. Meanwhile, the proposed unbiased prediction does one more thing, thinking about ``what if'' during inference. What if the ``riding'' between man and surfboard is not activated, their relationship could simply be ``on'' or ``above''. Based on such a counterfactual thinking~\cite{Judea2018thebookofwhy}, the changing of likelihood from the unactivated ``man'' and ``surfboard'' to the real activated ``man riding surfboard'' is used as the indicator of unbiased SGG. Each ``what if'' will be individually identified reflecting indirect bias of corresponding subject-object pair.

% Actually, the above mentioned counterfactual thinking~\cite{Judea2018thebookofwhy} is the individual version of the randomized controlled trial (RCT)~\cite{chalmers1981method}, which is regarded as the golden rule to conduct unbiased scientific experiments. Benefit from the hindsight, even if we can't simultaneously conduct treatment and untreatment to the same individual, counterfactual thinking helps us imagine ``what if'' in our brains, so the real case and what-if case could serve as experimental group and control group as in RCT.

% Inspired by such a counterfactual thinking of human beings, an unbiased SGG can be defined as which predicate would have been suppressed if the detailed subject-object information was erased and everything else (entity labels and background environment) had been the same. This definition can also be called as the total direct effect in effect analysis~\cite{vanderweele2015explanation, vanderweele2013three, pearl2001direct, robins1992identifiability}. As shown in Figure~\ref{fig:2}, we illustrate the difference between the conventional static likelihoods and the total direct effect~\cite{vanderweele2013three, vanderweele2015explanation} of subject-object signals. The bottom of Figure~\ref{fig:2}.b is the causal graph version of the proposed effect analysis. Causal graph~\cite{pearl2016causal} is a directed structural model indicating how factors of interest interact with each other, which helps us distinguish the direct effects from other indirect ones.  

% Our contributions can be concluded into three folds: 1) this paper firstly applies effect analysis to SGG that significantly improves the mean Recall@K~\cite{tang2019learning, chen2019knowledge} and zero-shot Recall@k in Visual Genome~\cite{krishna2017visual}. Although we observe a performance drop on conventional Recall@k, a deeper analysis shows that only several superclasses of predicate get decreased while the corresponding subclasses have significantly improvements, which suggests that the drop is caused by the more fine-grained SGG. 2) The proposed direct effect generation is model-agnostic. We observe similar improvements on VTransE~\cite{zhang2017visual}, MOTIFS~\cite{zellers2018neural} and VCTree~\cite{tang2019learning}. 3) To fully evaluate the value of generated SG for downsteam tasks, we introduce the image caption-to-SG retrieval as the measurement. Unlike VQA~\cite{teney2017graph, antol2015vqa} or Captioning~\cite{yang2019auto, you2016image} that relies more on features and attentions than scene graphs. The proposed image caption-to-SG retrieval takes SGs as the only descriptions of images, hence it directly reflects the uniqueness and integrality of SGs towards corresponding images.



% Conditional on the rest factors, the direct effect measures the changing of likelihoods when the causal signal vary from unactivate to activate status. Causal graph~\cite{} is also required to analyze the causal relations among involved variables and further distinguish the direct effect from indirect effect. It's also easy to point out that the causal signal in SGG is the subject-object entity features. For example, without the legs crossing the horseback, the man is not riding the horse.

%Image is not just the combination of objects. It also provides an organic environment of how objects relate to each other and interact with each other. Scene Graph(SG)~\cite{Johnson_2015_CVPR} is introduced as such an abstraction of images. Recent works~\cite{shi2019explainable, yang2019auto, krishna2018referring} show that Scene Graph is important to high-level vision tasks as it provides a symbolic structure to conduct explicit and explainable reasoning among objects. However, before we take SG as the indispensable requirement towards downstream visual reasoning tasks, the reliability of Scene Graph Generation(SGG) is still questioned. The main challenge is due to the exponentially increased searching space of $\mathcal{O}(N^2M)$ triplet combinations for $N$ objects and $M$ predicates. Recent approaches reduce it to $\mathcal{O}(N+M)$ by individually predicting objects and predicates. Since each predicate itself is hard to memorize all $\mathcal{O}(N^2)$ types of patterns, the embedding of subject and object features will be provided~\cite{lu2016visual, zhang2017visual, zellers2018neural}, which causes a new type of co-occurrence bias. Due to the nature of end-to-end training, we can never make sure what our model will learn from the pair of subject-object features. According to the thorough investigation of Zellers~\etal's work~\cite{zellers2018neural}, a shortcut is revealed in SGG. They found that without even taking a look at the image, a blind model can infer predicates quite well by selecting the most likely predicate according to the statistics of subject-predicate-object combinations across the dataset. Take an intuitive example, if 99\% percent of the relationship between the human and the horse is "riding" in the dataset. A model trained on this dataset is very likely to take the co-occurrence of human and horse as the shortcut for the riding predicate, rather than rely on the more complicated visual signals that "human on horse" and "legs cross horseback". We further confirm this conjecture by taking a deep look into the predicate prediction of a widely accepted framework: Neural-MOTIFS~\cite{zellers2018neural}. As illustrated in Figure~\ref{fig:1}~(b,c) We found that the overall prediction distribution is very similar to the distribution of corresponding statistical bias term. In statistics, XX\% of the predictions agree with the bias term while only XX\% of them predict are the same as their visual term. Such a bias causes the result that the frequent predicates are more easy to be predicted simply by blind guessing. This phenomenon is also noticed by Tang~\etal~\cite{tang2019learning} and Chen~\etal~\cite{chen2019knowledge}. They found that previous methods only work well on several frequent predicates while ignore the rest. In Figure~\ref{fig:1}(e), take MOTIFS~\cite{zellers2018neural} as an example, the Recall of tail predicates are nearly zeros. Therefore, recent SGG methods mainly contribute a relationship graph to downstream tasks rather than the specific meaningful predicates.

%Unlike most of the other biased task, \ie, texture bias to object classification~\cite{}, statistical bias in SGG does provide a meaningful prior. Object and subject categories are able to limit the capability of different entities. For instance, if an apple is on the horseback, we would say \textit{"apple on horse"} rather than \textit{"apple riding horse"}. Methods like weighted cross entropy loss will falsely encourage the extreme cases and distort these commonsense. 3) Disentangle the biased representation is also not straightforward. If we remove the statistical prior term in the first place, we will get a contaminated model, which is like fitting $y=2x+3$ with the model $y=kx$. Meanwhile, If we remove the statistical prior term after the training, the meaningful prior is also lost together with the bias term, not to mention that we can never make sure the successful disentanglement in an end-to-end trained model without any constraint.

%To sum up, the statistical bias itself is not the problem, which is also naturally existing in human intelligence. Part of our human commonsense is based on the co-occurrence of certain entities. The real problem is that the bias takes the place of the real causal signals, \ie, the visual feature of entities, and becomes the dominating cause of the predicate categories. Meanwhile, despite the fact that our human beings are also exposed to a biased world, we will not misclassify the "ambulance" even if they are less frequent than normal cars. Actually, our human beings can even benefit from biased prior knowledge by filtering impossible outcomes. The main difference is that human intelligence allows us to focus on the effect of real causal signals, \ie, shape to object categories, entity status to relationships. 

%Based the above mentioned problems, we introduce effect analysis as the remedy for SGG. As we mentioned above, the main advantage of human intelligence is to focus on the causal signals. Although the causal signal varies from task to task, it's easy to point out that the causal signal in SGG is subject-object entity features. For example, without the legs crossing the horseback, the man is not riding the horse. To identify the causal effect, the capability of thinking "without" is required. In Figure~\ref{fig:2}, we illustrate the difference between the conventional static logits from a fully connect prediction layer and the direct effect of causal signals. Conditional on the rest factors, the direct effect measures the changing of predictions when the causal signal vary from unactivate to activate status. Since causal graph is direct related towards the network structures, it's very easy to conduct effect analysis in SGG as a postprocessing.

%Our contributions can be concluded into three folds: 1) the proposed postprocessing of effect analysis significantly improves the mean Recall@K~\cite{tang2019learning, chen2019knowledge} and zero-shot Recall@k in Visual Genome~\cite{}. Although we observe a performance drop on conventional Recall@k, a further analysis shows that only several superclasses of predicate get decreased while the corresponding subclasses have significantly improvement, which implies the fact that the drop is caused by the more finegrained SG. 2) The proposed effect analysis is also model-agnostic. We observe similar improvements under VTransE~\cite{}, MOTIFS~\cite{zellers2018neural} and VCTree~\cite{tang2019learning}. 3) To evaluate the value of generated SG for downsteam tasks, we introduce a captioning-to-SG image retrieval task to test the generated SG. Unlike VQA or Captioning that relies more on features and attentions than scene graph based reasoning. The captioning-to-SG image retrieval is better describe the value of SG as the abstraction of images, because it only rely on how a generated SG can be integratedly and uniquely describe the image.

%Teaser figure. top: Biased training +biased testing (conventional) p(y|x) beneath the arrow. show drawback 1) on/near too many, 2) z's bias。 bottom: unbiased sgg (ours) effect analysis beneath the arrow, show our qualitative example, removing the above two biases.

% Biased Tr + Biased Te bad

%2. All due to the bias. two kinds of biases: selection bias (need survey, tend to give simple, general annotation rather than specific annotation) (on), language bias (z). x->y, z->y. All existing model explicitly exploit such bias, why benefit? 

% UnBiased Tr + UnBiased Te bad,  1) expensive 2) SGG needs language bias
% How to directly attack? for bias 1, can use line1: balanced sample, obvious predicate no annotation, missed? balance-->more cost, never enough prohibitively expensive.  for bias 2, use weighted softmax --> just a penalty for frequency predicates, still a fixed statistical solution for all cases? not case by case analysis whether it is biased. 

% if remove them, we will have 1) y = kx+b. 2) no respect to prior knowledge. (wiki why model prior is important for training).

% Biased Tr + Unbiased Te good
%Though we respect biased training, reasoning cannot use LIKELIHOOD. Human = Learning + Reasoning. if still use likelihood to generate, then like the begining, the biased model will predict biased sg, rare class, (zero-shot)。 

%Biased Tr + Unbiased Te (intuitive way) bad.
%我们的核心是：减掉改减去的bias vs 减掉了不该剪去的bias， 减掉物体pair没参与的bias vs 减掉物体pair原本存在的bias
%(related work) Current bias removal model can be categorized into two lines of bias removal methods (DO DOUBLE-CHECK) 1) balanced samples, 2) loss.  Essentially, they all disrespect the nature of the data. 

%So, why dont we respect the biased training, and infer the relationship from the biased model? Mention human intelligence: 我们人的推理总能鱼和熊掌兼得，即享受context和z的便利，但又不被他们束缚. So, rethink the contribution of the 3 key ingredients: x, z, c. 

%Mediation analysis to disentangle the highly nonlinear model in PRINCIPLED, THEORECTICAL FRAMEWORK. 1) Given a causal graph, 2) training, 3) effect. We will never bother to cost on data annotation, not the guilty data, but our prediction.   (discuss the benefit of biased training or not?)

%\subsection{Causal Graph}

%One of the most significant difference between causality and statistics is that causality requires a directed causal graph while statistics only reveals undirected correlation. As the foundation for most of the causal analysis methods, causal graph is a manually defined prior structure shows how interested variable are interacted toward final outcomes. Note that even the design of causal graph is purely dependant on designers, a wrong or worse causal graph still can be identified. As the wrong causal graph doesn't reveal the inherent interaction among interested variables, the fitted model tends to perform bad in test set. The evolution of more precise causal graphs is behind the evolution of scene graph generation frameworks, even most of the researchers didn't realize. The causal graph used in this paper is adopted from recent state-of-the-art methods~\cite{zellers2018neural, tang2019learning, chen2019counterfactual}, which best describe the underline relationship among object features, object labels, image context and predicate labels.

%\subsection{Image Retrieval Based on Scene Graph, Delete?}
%Most of the existing image retrieval methods~\cite{rui1999image, liu2007survey} only focus on instance-centric image retrieval, which limits the power of finding semantically similar images. There are several works~\cite{Johnson_2015_CVPR, schuster2015generating} trying to utilize scene graph for better semantic image retrieval. \cite{Johnson_2015_CVPR} introduces the notion of the scene graph and use it to retrieve images. \cite{schuster2015generating} further provides a solution to generate scene graph from text description, which is closer to user habits. However, those methods use SGs as the queries rather than the representations of images. To evaluate how a generated SG can uniquely and integrally represent the image. We introduce Image Caption-to-SG Retrieval in Section~\ref{sec:retrieval}.

%\subsection{Effect Analysis}
%There are three types of effect in causal effect analysis~\cite{vanderweele2015explanation, vanderweele2013three, pearl2001direct}: Total Effect (TE), Direct Effect (DE) and Indirect Effect (IE). The later two can also be divided into Total/Natural Direct Effect (TDE/NDE) and Total/Natural Indirect Effect (TIE/NIE). IE and DE correspond to the paths with and without mediator respectively, \ie, $A\to M\to B$ and $A\to B$ in Figure~\ref{fig:5}~a. TE takes both two paths into account. In any system with mediators (linear or nonlinear), $TE = TDE + NIE = NDE + TIE$. In linear system, there is no difference between TDE and NDE or TIE and NIE. In nonlinear system, the effect containing nonlinear interactions between DE and IE is called TDE/TIE, while the effect without interactions is called NDE/NIE or Pure Direct Effect/ Pure Indirect Effect (PDE/PIE) in \cite{vanderweele2013three}. To successfully decompose the TE, the interaction should be either put in DE or IE.

%To generate unbiased SG, we utilize TDE of the subject-object visual features $X$ during inference, because it's the causal signal of predicate categories. The TDE is calculated under the environment/context $u$, which is the entire image contains the feature map $m$ and all bounding boxes $B$ detected by a pretrained detector. Both TE and the NIE are not chosen, because they are affected by non-causal signals that may contain bias. In our case, TE, NIE and NDE can be calculated as following:
%\begin{align}
%TE(X|u) &= Y(X,Z,u) - Y(X^*,Z^*,u), \label{eq:1} \\
%NIE(X|u) &= Y(X^*,Z,u) - Y(X^*,Z^*,u), \label{eq:2} \\
%TDE(X|u) &= TE - NIE \label{eq:3} \\
%    &= Y(X,Z,u) - Y(X^*,Z,u), \label{eq:4}
%\end{align}
%where $X^*$ indicates the unactivated subject-object features and $Z^*$ is the corresponding $Z$ generated from $X^*$, $Y(\cdot)$ represents the entire framework introduced in the next subsection that outputs a set of pairwise predicates ${y_{ij}}$. 







%\begin{table*}
%\centering
%\scalebox{.8}{
%\begin{tabular}{l | c c|c c|c c}
%\hline
%\multicolumn{1}{c}{} & \multicolumn{2}{c}{Scene Graph Detection} & \multicolumn{2}{c}{Scene Graph Classification} & \multicolumn{2}{c}{Predicate Classification} \\
%\hline
%Model & R@20~/~50~/~100 & mR@20~/~50~/~100 & R@20~/~50~/~100 & mR@20~/~50~/~100 & R@20~/~50~/~100 & mR@20~/~50~/~100  \\ 
%\hline 
%IMP+~\cite{xu2017scene, chen2019knowledge} & 14.6~/~20.7~/~24.5 & -~/~3.8~/~4.8 & 31.7~/~34.6~/~35.4 & -~/~5.8~/~6.0 & 52.7~/~59.3~/~61.3 & -~/~9.8~/~10.5 \\
%FREQ~\cite{zellers2018neural, tang2019learning} & 20.1~/~26.2~/~30.1 & 4.5~/~6.1~/~7.1 & 29.3~/~32.3~/~32.9 & 5.1~/~7.2~/~8.5 & 53.6~/~60.6~/~62.2 &  8.3~/~13.0~/~16.0 \\
%MOTIFS~\cite{zellers2018neural, tang2019learning} & 21.4~/~27.2~/~30.3 & 4.2~/~5.7~/~6.6 & 32.9~/~35.8~/~36.5 & 6.3~/~7.7~/~8.2 & 58.5~/~65.2~/~67.1 & 10.8~/~14.0~/~15.3 \\
%KERN~\cite{chen2019knowledge} & -~/~27.1~/~29.8 & -~/~6.4~/~7.3 & -~/~36.7~/~37.4 & -~/~9.4~/~10.0 & -~/~65.8~/~67.6 & -~/~17.7~/~19.2 \\
%VCTree~\cite{tang2019learning} & 22.0~/~27.9~/~31.3 & 5.2~/~6.9~/~8.0 & 35.2~/~38.1~/~38.8 & 8.2~/~10.1~/~10.8 & 60.1~/~66.4~/~68.1 & 14.0~/~17.9~/~19.4\\
%\hline 
%MOTIFS\textsuperscript{$\dagger$} & 25.1~/~32.1~/~36.9 & 4.1~/~5.5~/~6.8 & 35.8~/~39.1~/~39.9 & 6.5~/~8.0~/~8.5 & 59.5~/~66.0~/~67.9 & 11.5~/~14.6~/~15.8 \\
%MOTIFS\textsuperscript{$\dagger$}-TestX & - & - & - & - & - & - \\
%MOTIFS\textsuperscript{$\dagger$}-TrainX & - & - & - & - & - & - \\
%MOTIFS\textsuperscript{$\dagger$}-WeightedCE & - & - & - & - & - & - \\
%MOTIFS\textsuperscript{$\dagger$}-TE & - & - & - & - & - & - \\
%MOTIFS\textsuperscript{$\dagger$}-TIE & - & - & - & - & - & - \\
%MOTIFS\textsuperscript{$\dagger$}-TDE & 12.4~/~16.9~/~20.3 & 5.8~/~8.2~/~9.8 & 21.7~/~27.7~/~29.9 & 9.8~/~13.1~/~14.9 & 33.6~/~46.2~/~51.4 & 18.5~/~25.5~/~29.1 \\
%MOTIFS\textsuperscript{$\dagger$}-TDE-Zero & - & - & - & - & - & - \\
%\hline
%MOTIFS\textsuperscript{$\dagger$}-RUBi & 25.8~/~33.3~/~37.8 & 5.2~/~7.2~/~8.5 & 36.2~/~39.4~/~40.1 & 7.2~/~9.0~/~9.5 & 58.9~/~65.5~/~67.4 & 12.2~/~15.5~/~16.8\\
%MOTIFS\textsuperscript{$\dagger$}-RUBi-TDE & 5.9~/~7.4~/~8.4 & 6.6~/~8.5~/~9.9 & 21.8~/~27.2~/~29.5 & 11.1~/~13.9~/~15.2 & 38.7~/~50.8~/~55.8 & 18.5~/~24.9~/~28.3\\
%\hline
%VTransE\textsuperscript{$\dagger$} & 23.0~/~29.7~/~34.4 & 3.7~/~5.0~/~6.0 & 35.4~/~38.6~/~39.4 & 6.7~/~8.2~/~8.7 & 59.0~/~65.7~/~67.6 & 11.6~/~14.7~/~15.8 \\
%VTransE\textsuperscript{$\dagger$}-TDE & 13.5~/~18.7~/~22.6 & 6.3~/~8.6~/~10.5 & 19.7~/~25.7~/~28.5 & 9.3~/~12.9~/~14.8 & 36.9~/~48.5~/~53.1 & 17.3~/~24.6~/~28.0 \\
%\hline
%VTransE\textsuperscript{$\dagger$}-RUBi & 24.5~/~31.3~/~35.5 & 5.1~/~6.8~/~8.0 & 34.6~/~38.1~/~38.9 & 6.6~/~8.2~/~8.7 & 58.7~/~65.3~/~67.1 & 13.6~/~17.1~/~18.6 \\
%VTransE\textsuperscript{$\dagger$}-RUBi-TDE & 13.7~/~19.0~/~22.9 & 6.0~/~8.5~/~10.2 & 23.0~/~28.8~/~31.1 & 9.8~/~13.1~/~14.7 & 40.0~/~50.7~/~54.9 & 18.9~/~25.3~/~28.4\\
%\hline
%VCTree\textsuperscript{$\dagger$} & 24.7~/~31.5~/~36.2 & 4.2~/~5.7~/~6.9 & 37.0~/~40.5~/~41.4 & 6.2~/~7.5~/~7.9 & 59.8~/~66.2~/~68.1 & 11.7~/~14.9~/~16.1 \\
%VCTree\textsuperscript{$\dagger$}-TDE & 14.0~/~19.4~/~23.2 & 6.9~/~9.3~/~11.1 & 19.9~/~25.4~/~27.9 & 8.9~/~12.2~/~14.0 & 36.2~/~47.2~/~51.6 & 18.4~/~25.4~/~28.7 \\
%\hline
%VCTree\textsuperscript{$\dagger$}-RUBi & 24.8~/~31.8~/~36.1 & 4.9~/~6.6~/~7.7 & 35.4~/~38.9~/~39.8 & 6.3~/~7.5~/~8.0 & 59.1~/~65.5~/~67.4 & 12.4~/~15.4~/~16.6 \\
%VCTree\textsuperscript{$\dagger$}-RUBi-TDE & 14.3~/~19.6~/~23.3 & 6.3~/~8.6~/~10.3 & 22.8~/~28.8~/~31.2 & 8.9~/~11.8~/~13.4 & 39.1~/~49.9~/~54.5 & 17.2~/~23.3~/~26.6 \\
%\hline
%\hline
%\end{tabular}
%}
%\caption{The reimplemented SGG models under our detector and hyper-parameters are denoted by the superscript \textsuperscript{$\dagger$}. }
%\label{tab:1}
%\end{table*}



%We argue that the main cause of the biased prediction is because the existing methods are incapable of separating the effect of causal signals from other inputs and underlying model preferences, \eg, separating the fraction of logits that caused by 'the legs crossing the horseback' from the co-occurrence of 'horse' and 'person' given 'person riding horse'. Benefit from the development of the causal inference~\cite{Judea2018thebookofwhy, pearl2016causal, vanderweele2015explanation}, we are now able to obtain the unbiased causal effects through mediation analysis~\cite{vanderweele2015explanation, vanderweele2013three, pearl2001direct}. To conduct mediation analysis, we have to perform surgeries on the causal graph~\cite{Judea2018thebookofwhy, pearl2016causal} then extract the effect that is directly caused by the appearance of causal signals. Note that the effects of inputs towards predicates are considered as logits in this paper. 

%Before we dive into the specific case of TDE for the above SGG framework, we briefly review the concepts of \textit{do} operation, counterfactual reasoning, mediator and three types of causal effects.

%\noindent\textbf{\textit{do} Operation}. \textit{do} operation is defined as a type of intervention that forces one or more variables in the causal graph to take certain values. For example,  in a study of the gender discrimination in job-hunting, we try to identify the result of a applicant when all the backgrounds are kept the same but change gender to $female$, \ie, $\textit{do}(\text{Gender}=female)$. \textit{do} operation can also be considered as perform a surgery on the causal graph that wipes out all the in-coming links of the variable, so the value is directly assigned rather than dependent on ancestor nodes. 

%\noindent\textbf{Counterfactual Reasoning}. Equipped with \textit{do} operation, we are now able to conduct counterfactual reasoning: imagining the output of certain value combination of variables that never been observed. In our case, given an image $I=u$ (\ie, a situation), we use $Y_x(u)$ to denote the logits of $Y$ that obtained under $do(X=x)$, and $Y_{x,z}(u)$ when two variables are controlled by $do(X=x)$, $do(Z=z)$.

%\noindent\textbf{Mediator}. In a causal graph, when we care about the effect of a variable to another, the descendant node of the former variable that is located between the path of two is a mediator. In our case, variable $Z$ is the mediator of $X$ to $Y$, which can be considered as the side effect of $X$ that also affects $Y$. 

%For example, in the study of carcinogenesis by smoke ($\text{Cigarette}\to \text{Nicotine}\to \text{Cancer}$), nicotine is a mediator. 

%\noindent\textbf{Total Effect (TE)}. TE measures the increase of output $Y$ when the treatment variable changes from unactivated to activated. In Figure~\ref{fig:4}(b), TE of pairwise object feature $X$ can be formulated as:
%\begin{equation}
%    TE=Y_{x}(u) - Y_{\bar{x}}(u),
%    \label{eq:te}
%\end{equation}
%where $\bar{x}$ indicates the unactivated value of $X$ that can be either mean feature on the training set or simply zero vector. Since the intervention is only conducted on $X$ leaving the input arrow of $Z$ untouched, the current value of $Z=\bar{z}$ is calculated from $X\to Z$, taking $\bar{x}$ as input.

%\noindent\textbf{Natural Indirect Effect (NIE)}. NIE (\textit{a.k.a.} Pure Indirect Effect) measures the portion of TE that would be transmitted to $Y$ responding to the change of $Z$ when the effort of $X$ is absent. 
%\begin{equation}
%    NIE=Y_{\bar{x},z}(u) - Y_{\bar{x},\bar{z}}(u).
%    \label{eq:nie}
%\end{equation}

%\noindent\textbf{Total Direct Effect (TDE)}. TDE measures the remaining portion of TE when NIE is removed. It can be calculated as:
%\begin{equation}
%    TDE=TE-NIE=Y_{x,z}(u) - Y_{\bar{x},z}(u).
%\end{equation}
%$Y_{\bar{x}}(u)$ is equal to $Y_{\bar{x},\bar{z}}(u)$ based on the definition of $\bar{z}$.

%In SGG, the predicate is only confirmed when the pairwise object is seen. Hence, we are interested in the path $X\to Y$, \ie, the TDE of $X$. The counterfactual term $Y_{\bar{x},z}(u)$ removed from logits is equivalent to the model bias out of a blind guess. The experimental analysis of TE, NIE, TDE is conducted in Section~\ref{sec:exp}.

%In this section, we use cause-effect analysis for unbiased prediction. Mediation analysis. 
%1. We are only interested in the path X --- Y. That is, the direct effect. mention that the effect is considered as logit here.
%2. Full formulation of tde, start from the do operation for counterfactuals, with a change.




\section{Image Caption-to-SG Retrieval}
\label{sec:retrieval}
 SG-based VQA~\cite{teney2017graph, shi2019explainable} and Captioning~\cite{yang2019auto, yao2018exploring} rely more on hidden features and attentions than SGs. Even SG based image retrieval~\cite{Johnson_2015_CVPR} only utilizes SGs as queries and still using hidden features to represent images. The proposed image Caption-to-SG retrieval firstly considers SGs as the sole representations of images, the same as how we wish it serving downstream tasks. The performance of image Caption-to-SG retrieval can be used to measure the uniqueness and integrality of how a generated SG matches the human description towards the image. 

\subsection{Task Definition}
We select 41,859 images that contain coco caption annotations~\cite{lin2014microsoft} from VG dataset~\cite{krishna2017visual}, and separate them into three sets, train/test-1k/test-5k $(35,859/1,000/5,000)$, where the later two both selected from the VG test set. Ground truth captions are used to retrieve the generated SGs (SGDet) containing entities $E=\{e_i\}$ and relationships $R=\{r_{ij}=(s_i,p_{ij},o_j)\}$. To simplify the problem, for each image, all annotated captions are merged together to generate one text-SG by a SG-parser~\cite{schuster2015generating}. The problem is then transformed into comparing the similarity of text-SGs and image-SGs. The embedding method adopted in our work is BAN~\cite{kim2018bilinear}, which will be introduced in the next subsection. L1 distance with triplet loss~\cite{schroff2015facenet} is used to train the embedding model of SG. 

\subsection{Bilinear Attention Scene Graph Embedding}
Since entities and relationships are both important for SGs, we apply Bilinear Attention Network (BAN)~\cite{kim2018bilinear} to encode their multimodal interactions into the same representation space.

Different embedding layers are used for text-SGs and image-SGs with vocabularies $k\in\{text, image\}$. The entities and relationships are embedded as $E_{embed}^k=W_e^k E^k$, $R_{embed}^k=[W_s^k S^k; W_p^k P^k; W_o^k O^k]$, where $E_{embed}^k\in \mathbb{R}^{N_d \times N_e^k}$, $R_{embed}^k \in \mathbb{R}^{3N_d \times N_r^k}$, $N_e^k, N_r^k$ are numbers of entities and relationships for each image, $P^k, E^k, S^k, O^k$ represent onehot vectors of predicates, entities, subjects and objects respectively, and the later three share the same vocabulary under each $k$.

The same BAN model is used for both text-SGs and image-SGs, hence we remove $k$ below for simplification. The original BAN involves two steps: 1) attention map generation, and 2) bilinear attended feature calculation. Since scene graph has already given connections between entities and relationships, we skip the first step and use normalized scene graph connection as attention map $A_{ij}=M_{ij} / \sum_j M_{ij}$, where $A,M\in \mathbb{R}^{N_e \times N_r}$, the scene graph connection $M$ is defined as follows:
\begin{equation}
    M_{ij}= \left\{
    \begin{aligned}
        1 &,\ if\ E_i\ in\ R_j,\\
        0 &,\ if\ E_i\ not\ in\ R_j.
    \end{aligned}
    \right.
\end{equation}

The bilinear attended feature vector is calculated as $f=BAN(E_{embed}, R_{embed}; A)=W_b c$, where $W_b\in \mathbb{R}^{N_d \times N_p}$, $c\in \mathbb{R}^{N_p}$ and the $p^{th}$ element of $c$ is calculated as:
\begin{equation}
    c_p=\sum_{i=1}^{N_e} \sum_{j=1}^{N_r} A_{ij} (E_{embed})_i^T ((W_e)_p(W_r)_p^T) (R_{embed})_j,
\end{equation}
where $W_e\in \mathbb{R}^{N_d \times N_p}, W_r\in \mathbb{R}^{3N_d\times N_p}$.

The multi-layer version of BAN can be further defined in the form of residual addition:
\begin{equation}
    F_{i+1} = BAN_i(F_i, R_{embed}; A)\cdot \mathbf{1}^T + F_i,
\end{equation}
where $F_0 = E_{embed}$. The eventual embedding of the entire SG is $SG_{embed}=mean(F_R), SG_{embed}\in \mathbb{R}^{N_d}$ if we set number of residual layers to $R$.

